Impact of misalignments on the analysis of B decays

This note investigates the effects of a misaligned tracking system on the analysis of B decays. Misalignment effects of both the vertex locator and the inner and outer T-stations have been studied. $z$-scaling effects of the vertex locator are also considered. It is proven that misalignments of the order of the detector single-hit resolutions have little or negligible effects on the quality of the reconstruction and of the analysis of B decays. The studies were performed with a sample of $B^0_{(s)} \to h^+h^{'-}$ decays, but the impact of misalignments on the performance of the pattern recognition algorithms and on the primary vertex resolutions, assessed for the first time, are rather general and not restricted to $B^0_{(s)} \to h^+h^{'-}$ decays.

==> mysettings.tex <==
% ----------------
% Packages to load
% ----------------
% A load of standard graphics commands
\usepackage[dvips]{graphics}  % standard graphics commands
\usepackage{epsfig}     % EPS manipulation with \epsfig
%\usepackage{psfig,epsfig}     % EPS manipulation with \epsfig
\usepackage{amssymb,latexsym}
\usepackage{latexsym}         % extra maths symbols
\usepackage{indentfirst}      % identation also on 1st paragraph of a section
\usepackage{alltt}
\usepackage{fancyhdr}
\usepackage{supertabular}

% -------------
% Page settings
% -------------
\renewcommand{\baselinestretch}{1.2}
\def\dline{ \renewcommand{\baselinestretch}{1.5}
            \small
            \normalsize
          }
\def\sline{ \renewcommand{\baselinestretch}{1}
            \small
            \normalsize
          }

% ------------------------------
% Space above and below formulae
% ------------------------------
\addtolength{\abovedisplayskip}{1mm}
\addtolength{\belowdisplayskip}{1mm}
\addtolength{\abovedisplayshortskip}{1mm}
\addtolength{\belowdisplayshortskip}{1mm}


%--------------------
% Horizontal spacings
%--------------------
\setlength{\hoffset}%
          {-1.in}
\setlength{\evensidemargin}{2.5cm}
\setlength{\oddsidemargin}{3.0cm}
\setlength{\textwidth}{\paperwidth}
\addtolength{\textwidth}{-\evensidemargin}
\addtolength{\textwidth}{-\oddsidemargin}
%------------------
% Vertical spacings
%------------------
\setlength{\voffset}{-0.5cm}
\setlength{\topmargin}{0.5cm}
\setlength{\headheight}{0.5cm}
\setlength{\headsep}{0.5cm}
\setlength{\footskip}{1.0cm}
\newlength{\footmargin}
\setlength{\footmargin}{2.0cm}
\setlength{\textheight}{\paperheight}
\addtolength{\textheight}{-1.in}
\addtolength{\textheight}{-\voffset}
\addtolength{\textheight}{-\topmargin}
\addtolength{\textheight}{-\headheight}
\addtolength{\textheight}{-\headsep}
\addtolength{\textheight}{-\footskip}
\addtolength{\textheight}{-\footmargin}
%-----------------
% Float parameters
%-----------------
\setlength{\floatsep}{6pt plus 3pt minus 1pt}
\setlength{\textfloatsep}{10pt plus 5pt minus 3pt}
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.9}
\renewcommand{\textfraction}{0.1}

%--------------------------------
% Settings for package "fancyhdr"
%--------------------------------
\pagestyle{fancy}
\lhead{}
\rhead{}
\cfoot{\bfseries \thepage}
%\lhead{\bfseries \slshape E. Rodrigues}
%\rhead{\bfseries \slshape Meeting, $1^{st}$ January 2003}
%\cfoot{\bfseries \slshape Some Title}
\renewcommand{\headrulewidth}{0.7pt}
\renewcommand{\footrulewidth}{0.7pt}

